POPT: Physics-Informed Deep Learning for Phase-Only Positioning in Distributed MIMO

This article develops a physics-informed deep learning framework for single-snapshot 3D phase-only positioning in narrowband phase-coherent distributed multiple-input multiple-output (D-MIMO) networks under two-ray propagation. Unlike prior phase-coherent D-MIMO localization methods that largely assume line-of-sight (LoS)-only channels, we consider a LoS path and a specular ground reflection. Since the narrowband single-snapshot observation cannot resolve these components in delay, their coherent superposition induces structured perturbations in the carrier phase measurements. To address this, we develop a Gaussian process (GP)-based model that learns the quasi-periodic phase distortion caused by ground reflection from carrier phase measurements collected at a small number of training locations and uses it to generate high-quality synthetic samples. Building on these samples, we propose the Phase-Only Positioning Transformer (POPT), an encoder-only transformer that captures inter-antenna point (AP) phase relationships without solving the highly non-convex maximum-likelihood (ML) problem underlying model-based estimators. We also derive the fundamental position error bound (PEB) and develop maximum-likelihood estimation (MLE) for the considered multipath phase-only D-MIMO positioning problem. Numerical results show that, with only 50 GP training locations, the proposed method achieves near-PEB accuracy. The analytical MLE is highly sensitive to relative permittivity mismatch, whereas the proposed method mitigates this dependence by learning the phase perturbation directly from measurement data. Compared with MLE, the proposed approach also reduces floating-point operation (FLOP) complexity and inference time by about 1.7 and 3.6 orders of magnitude, respectively.

==> supplemental_material_final.tex <==
%\documentclass[lettersize,journal]{IEEEtran}
%\usepackage{amsmath,amsfonts,amssymb}
%\usepackage{bm}
%\usepackage{mathtools}
%\usepackage{algorithmic}
%\usepackage{algorithm}
%\usepackage{array}
%\usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
%\usepackage{textcomp}
%\usepackage{stfloats}
%\usepackage{url}
%\usepackage{verbatim}
%\usepackage{graphicx}
%\usepackage{cite}
%\usepackage[acronym]{glossaries}
%\usepackage{booktabs}
%\usepackage{multirow}
%\usepackage[hidelinks]{hyperref}
%\usepackage{bibentry}
%\usepackage{xr-hyper}
%\usepackage{microtype}
%\usepackage{xcolor}



%\makeglossaries
%\input{acronyms}

%\begin{document}

\setcounter{equation}{0}
\renewcommand{\theequation}{S\arabic{equation}}

\noindent{\Large\textbf{Supplementary Material:\vspace{2mm}\\``\textls[-5]{POPT: Physics-Informed Deep Learning for Phase-Only Positioning in Distributed MIMO}''}}

%\section*{Appendix}\\CRLB and PEB Derivation}
\vspace{6pt}

In this supplementary material, we derive the \gls{fim} of the channel parameters in Section~\ref{sec:channel_parameter_fim} and the transformation matrix, which is used to compute the \gls{fim} of the \gls{ue} state, in Section~\ref{sec:transformation_matrix}. We also provide the detailed mathematical expressions of the transformer encoder operations deferred from Section~\ref{subsubsec:encoder} in Section~\ref{sec:transformer_encoder_operations}.

\section{Channel Parameter FIM}\label{sec:channel_parameter_fim}

Let $\veta = [\phi, \alpha_1, \ldots, \alpha_M, \theta_1, \ldots, \theta_M]^\top$ denote the unknown channel parameter vector, for which the \gls{fim} is computed as
\begin{equation}\label{eq:channel_fim}
[\vJ(\veta)]_{ij} = \frac{2}{\sigma_w^2} \sum_{m=1}^{M} \Re \left \{
\frac{\partial \bar{y}_m^*}{\partial \veta_i}
\frac{\partial \bar{y}_m}{\partial \veta_j} \right \}, \:
i,j \in \{1,\ldots,2M+1\},
\end{equation}
where $\bar{y}_m = \sqrt{P} \alpha_{m}\exp{\left(-\jmath (\theta_{m} + \phi)\right)}s$ denotes the noise-free received signal. The \gls{fim} can be block-partitioned as follows
\begin{equation}
\vJ(\veta)=
\begin{bmatrix}
J_{\phi\phi}          & \vJ_{\phi\valpha}          & \vJ_{\phi\vtheta}\\
\vJ_{\valpha\phi}     & \vJ_{\valpha\valpha}       & \vJ_{\valpha\vtheta}\\
\vJ_{\vtheta\phi}     & \vJ_{\vtheta\valpha}       & \vJ_{\vtheta\vtheta}
\end{bmatrix},
\label{eq:FIM_block_partition}
\end{equation}
where $\valpha=[\alpha_1,\ldots,\alpha_M]^\top$ and $\vtheta=[\theta_1,\ldots,\theta_M]^\top$. The partial derivatives of $\bar{y}_m$ with respect to the channel parameters are 
\begin{equation}
    \frac{\partial \bar{y}_m}{\partial \phi} = -\jmath \bar{y}_m, \quad
    \frac{\partial \bar{y}_m}{\partial \alpha_{m'}} = \frac{\bar{y}_m}{\alpha_{m'}}, \quad
    \frac{\partial \bar{y}_m}{\partial \theta_{m'}} = -\jmath \bar{y}_m,
\end{equation}
in which $m' = m$, and otherwise the partial derivatives are
\begin{equation}
    \frac{\partial \bar{y}_m}{\partial \alpha_{m'}} = 0, \quad
    \frac{\partial \bar{y}_m}{\partial \theta_{m'}} = 0, \quad
    \text{if} \quad m \neq m'.
\end{equation}
Plugging the partial derivatives into \eqref{eq:channel_fim}, the block diagonal elements of the \gls{fim} are given by
\begin{subequations}
 \begin{align}
    J_{\phi\phi} &= \sum_{m=1}^M \frac{2P}{\sigma_w^2}  \alpha_m^2, \\
    \vJ_{\valpha\valpha}  &= \frac{2P}{\sigma_w^2}\vI_{M \times M}, \\
    \vJ_{\vtheta\vtheta}  &= \frac{2P}{\sigma_w^2} \diag([\alpha_1^2,\ldots,\alpha_M^2]). \label{eq:Jthetatheta}
\end{align}   
\end{subequations}
Respectively, the cross-elements of the \gls{fim} are given by
\begin{equation}
    \vJ_{\phi\valpha} = \mathbf{0}_{1 \times M}, \quad
    \vJ_{\phi\vtheta}  = \frac{2P}{\sigma_w^2} \valpha_{\text{sq}}^{\top}, \quad
    \vJ_{\valpha\vtheta}  = \mathbf{0}_{M \times M}.
\end{equation}
% \begin{subequations}
% \begin{align}
%     J_{\phi\valpha} &= \mathbf{0}_{1 \times M}, \\
%     \vJ_{\phi\vtheta}  &= \frac{2P}{\sigma_w^2} (\valpha^2)^\top, \\
%     \vJ_{\valpha\vtheta}  &= \mathbf{0}_{M \times M}.
% \end{align}
% \end{subequations}

\section{Transformation Matrix}\label{sec:transformation_matrix}

Next, we derive the transformation matrix, defined as 
\begin{equation}
[\vH_\vx(\vtheta)]_{m}
= \frac{\partial \theta_m}{\partial \vx}, \quad
m\in\{1,\ldots,M\}.
\end{equation}
By utilizing the definition of complex logarithm $\log z = \ln{\vert z \vert} + \jmath \arg{z} \Leftrightarrow \arg{z} = \Im\left\{ \log z \right\}$, the $m^{\text{th}}$ row of the Jacobian matrix can be written as 
\begin{subequations}
\begin{align} \label{eq:phase_diff}
\!\!\! \frac{\partial \theta_m}{\partial \vx} \!&=\! \Im \left\{ \frac{1}{\bar{y}_m} \frac{\partial \bar{y}_m}{\partial \vx} \right\} \\ \label{eq:phase_diff2}
&= \! \Im \left\{\frac{\sum_{i=1}^2 \! \left( \frac{\partial \alpha_m^{(i)}}{\partial \vx} \!-\! \jmath \alpha_m^{(i)} \frac{\partial \theta_m^{(i)}}{\partial \vx} \right)\exp(-\jmath\theta_m^{(i)}) }{\sum_{i=1}^2 h_m^{(i)}(\vx)}\right\},
\end{align}
\end{subequations}
where $\bar{y}_m = \sqrt{P}\big(h_m^{(1)}(\vx) + h_m^{(2)}(\vx) \big) \exp{(-\jmath\phi)}s$ is the received signal without noise.

The partial derivatives for the amplitude and phase of the LOS path can be straightforwardly obtained as
\begin{subequations}
\begin{align}
\frac{\partial \alpha_m^{(1)}}{\partial \vx} &= \frac{\lambda}{4\pi} \frac{\vdeltam^\top}{\Vert \vdeltam \Vert^3} \text{ and} \\
\frac{\partial \theta_m^{(1)}}{\partial \vx} &= -\frac{2\pi}{\lambda} \frac{\vdeltam^\top}{\Vert \vdeltam \Vert},
\end{align}
\end{subequations}
respectively, where $\vdeltam = \vp_m-\vx$. Furthermore, regarding the ground-reflected path, the corresponding partial derivatives of the amplitude and phase are given as
\begin{subequations}
\begin{align}
\frac{\partial \alpha_m^{(2)}}{\partial \vx} &= \frac{\lambda}{4\pi \Vert \vdeltamtilde \Vert} \left(\frac{\vert \Gamma_m(\vx)\vert \vdeltamtilde^\top}{\Vert \vdeltamtilde \Vert^2} + \frac{\partial \vert \Gamma_m(\vx)\vert}{\partial \vx}\right) \text{  and} \\
\frac{\partial \theta_m^{(2)}}{\partial \vx} &= -\frac{2\pi}{\lambda} \frac{\vdeltamtilde^\top}{\Vert \vdeltamtilde \Vert} - \frac{\partial \angle \Gamma_m(\vx)}{\partial \vx},
\end{align}
\end{subequations}
where $\vdeltamtilde = \tilde{\vp}_m-\vx$, and $\Gamma_m(\vx)$ is the reflection coefficient.

Considering the complex logarithm definition, used in \eqref{eq:phase_diff}, while exploiting the identities $\vert z \vert = \sqrt{z z^*}$ and $z + z^* = 2\Re\left\{ z \right\}$, the partial derivatives for the amplitude and phase of the reflection coefficient can be formulated as
\begin{subequations}
\begin{align}
\frac{\partial \vert \Gamma_m(\vx) \vert}{\partial \vx} &= \Re \left\{\frac{\Gamma_m^*(\vx)}{\vert \Gamma_m(\vx) \vert} \frac{\partial \Gamma_m(\vx)}{\partial \vx} \right\}\text{ and} \\
\frac{\partial \angle \Gamma_m(\vx)}{\partial \vx} &= \Im \left\{\frac{1}{\Gamma_m(\vx)} \frac{\partial \Gamma_m(\vx)}{\partial \vx} \right\},
\end{align}
\end{subequations}
respectively. After some algebraic manipulations, the complex-valued partial derivative of the reflection coefficient can be written as
\begin{align}
\frac{\partial \Gamma_m(\vx)}{\partial \vx} = \frac{2(1-\varepsilon_r)\sin(\gamma_m(\vx))}{\zeta(\vx)(\cos(\gamma_m(\vx)) + \zeta(\vx))^2} \frac{\partial \gamma_m(\vx)}{\partial \vx},
\end{align}
where %$\rho(\vx) = \cos(\gamma_m(\vx))$ and 
$\zeta(\vx) = \sqrt{\varepsilon_r - \sin^2(\gamma_m(\vx))}$. Furthermore, the partial derivative of the reflection angle reads
\begin{equation}
\frac{\partial \gamma_m(\vx)}{\partial \vx}
= -\frac{(z_m+z_{\textrm{ue}})\vdeltamtilde^\top + \left(d_m^{(2)}\right)^2 \mathbf{e}_3^\top}{\left(d_m^{(2)}\right)^3 \sqrt{1-\cos^2(\gamma_m(\vx))}},
%\left( \frac{z_{\textrm{ue}} + z_m}{d_m^{(2)}} \right)^2}}
\end{equation}
where $\mathbf{e}_3 = [0,0,1]^\top$.

% \begin{subequations}
% \begin{align}
%     \Gamma_m(\vx) &= \frac{\cos(\gamma_m(\vx)) - \sqrt{\varepsilon - \sin^2(\gamma_m(\vx))}}{\cos(\gamma_m(\vx)) + \sqrt{\varepsilon - \sin^2(\gamma_m(\vx))}} \\
%     &= \frac{\rho(\vx) - \zeta(\vx)}{\rho(\vx) + \zeta(\vx)}
% \end{align}
% \end{subequations}

%$\gamma_m(\vx) = \acos \left( \frac{z_{\textrm{ue}} + z_m}{d_m^{(2)}} \right)$


\section{Transformer Encoder Operations}\label{sec:transformer_encoder_operations}
The proposed encoder comprises $N_{\mathrm{enc}}$ stacked transformer encoder blocks that iteratively refine the token representations. Given the input representation $\mathbf{H}^{(0)}$ in \eqref{eq:final_popt_input}, the $q$-th encoder block, for $q\in\{1,\ldots,N_{\mathrm{enc}}\}$, adopts a pre-norm architecture expressed as


\begin{align}
\mathbf{Z}^{(q)} &= \mathrm{LN}\!\left(\mathbf{H}^{(q-1)}\right), \label{eq:enc_ln1}\\
\tilde{\mathbf{H}}^{(q)} &= \mathbf{H}^{(q-1)} + \mathrm{MHA}\!\left(\mathbf{Z}^{(q)}\right), \label{eq:enc_msa}\\
\mathbf{U}^{(q)} &= \mathrm{LN}\!\left(\tilde{\mathbf{H}}^{(q)}\right), \label{eq:enc_ln2}\\
\mathbf{H}^{(q)} &= \tilde{\mathbf{H}}^{(q)} + \mathrm{MLP}\!\left(\mathbf{U}^{(q)}\right), \label{eq:enc_ffn}
\end{align}
where the residual connections in \eqref{eq:enc_msa} and \eqref{eq:enc_ffn} maintain stable optimization by facilitating gradient propagation. \gls{ln} is defined for any vector $\mathbf{x}'$ as
\begin{equation}
\mathrm{LN}(\mathbf{x}')
=
\boldsymbol{\gamma}\odot
\frac{\mathbf{x}'-\mu(\mathbf{x}')}{\sqrt{\sigma^2(\mathbf{x}')+\epsilon}}
+\boldsymbol{\beta},
\end{equation}
where $\mu(\mathbf{x}')$ and $\sigma^2(\mathbf{x}')$ are the mean and variance of the entries of $\mathbf{x}'$, respectively, $\epsilon>0$ is a small constant, and $\boldsymbol{\gamma}$ and $\boldsymbol{\beta}$ are learnable vectors. In \eqref{eq:enc_ln1} and \eqref{eq:enc_ln2}, \gls{ln} is applied token-wise (row-wise) independently.

The \gls{mha} module computes queries, keys, and values through learned linear projections and, through its multi-head structure, allows the model to capture relationships in multiple representation subspaces. For head $h\in\{1,\ldots,N_{\mathrm{head}}\}$, the projections are
\begin{align}
\mathbf{Q}_{h}^{(q)} &= \mathbf{Z}^{(q)}\mathbf{W}_{Q,h}^{(q)}, \label{eq:Q_proj}\\
\mathbf{K}_{h}^{(q)} &= \mathbf{Z}^{(q)}\mathbf{W}_{K,h}^{(q)}, \label{eq:K_proj}\\
\mathbf{V}_{h}^{(q)} &= \mathbf{Z}^{(q)}\mathbf{W}_{V,h}^{(q)}, \label{eq:V_proj}
\end{align}
where
$\mathbf{W}_{Q,h}^{(q)},\mathbf{W}_{K,h}^{(q)},\mathbf{W}_{V,h}^{(q)}\in\mathbb{R}^{D_{\mathrm{emb}}\times d_h}$
are learnable weight matrices and $d_h=D_{\mathrm{emb}}/N_{\mathrm{head}}$ denotes the dimension of each attention head. The head output is computed using scaled dot-product attention as
\begin{equation}\label{eq:att_dot_prof}
\mathbf{A}_{h}^{(q)}=
\mathrm{softmax}\!\left(\frac{\mathbf{Q}_{h}^{(q)}\left(\mathbf{K}_{h}^{(q)}\right)^{\top}}{\sqrt{d_h}}\right)\mathbf{V}_{h}^{(q)}
\in\mathbb{R}^{M\times d_h},
\end{equation}
where $\mathrm{softmax}(\cdot)$ exponentiates each entry and normalizes each row independently. The scaling factor $1/\sqrt{d_h}$ prevents the inner products from growing excessively. Finally, the head outputs are concatenated and linearly transformed as
\begin{equation}\label{eq:mha}
\mathrm{MHA}\!\left(\mathbf{Z}^{(q)}\right)=
\!\left[\mathbf{A}_{1}^{(q)},\ldots,\mathbf{A}_{N_{\mathrm{head}}}^{(q)}\right]\mathbf{W}_{O}^{(q)},
\end{equation}
where $\mathbf{W}_{O}^{(q)}\in\mathbb{R}^{D_{\mathrm{emb}}\times D_{\mathrm{emb}}}$ is a learnable matrix.

The \gls{mlp} block in \eqref{eq:enc_ffn} is applied independently to each
row (token) of $\mathbf{U}^{(q)}$, and consists of two fully connected layers
with \gls{gelu} activation. For a row vector $\mathbf{u}\in\mathbb{R}^{D_{\mathrm{emb}}}$
corresponding to a single token, the MLP is defined as
\begin{equation}\label{eq:popt_mlp}
\mathrm{MLP}(\mathbf{u})=
\mathrm{GELU}\!\left(\mathbf{u}\mathbf{W}_{1}^{(q)}+\mathbf{b}_{1}^{(q)}\right)\mathbf{W}_{2}^{(q)}+\mathbf{b}_{2}^{(q)},
\end{equation}
where $D_{\mathrm{ff}}$ denotes the feed-forward hidden dimension, and
$\mathbf{W}_{1}^{(q)}\in\mathbb{R}^{D_{\mathrm{emb}}\times D_{\mathrm{ff}}}$
and $\mathbf{W}_{2}^{(q)}\in\mathbb{R}^{D_{\mathrm{ff}}\times D_{\mathrm{emb}}}$
are learnable weight matrices, while
$\mathbf{b}_{1}^{(q)}\in\mathbb{R}^{D_{\mathrm{ff}}}$ and
$\mathbf{b}_{2}^{(q)}\in\mathbb{R}^{D_{\mathrm{emb}}}$ are learnable bias vectors. After $N_{\mathrm{enc}}$ layers, the encoder output is $\mathbf{H}^{(N_{\mathrm{enc}})}\in\mathbb{R}^{M\times D_{\mathrm{emb}}}$, which is then passed to the Output Head described in the main text.


\section{Complexity Derivations for Benchmark Methods}\label{sec:benchmark_complexity}
The benchmark \gls{mlp} consists of seven hidden layers with widths $A,\,2A,\,4A,\,8A,\,4A,\,2A,$ and $A$, where $A=128$ as in~\cite{11275391}. The input dimension of the benchmark \gls{mlp} is $M-1$, corresponding to the differential phase measurements. Hence, the inference cost includes the input-to-hidden layer, the six hidden-to-hidden fully connected layers, and the output layer. The resulting complexity therefore scales as $\mathcal{O}_{\text{MLP}}=\mathcal{O}\!\left((M-1)A + A^2\right)$,
\begin{comment}
    \begin{equation}\label{eq:mlp_bigO}
\mathcal{O}_{\text{MLP}}=\mathcal{O}\!\left((M-1)A + A^2\right).
\end{equation}
\end{comment}
and the total number of \glspl{flop} can be approximated as~\cite{11275391} $\mathcal{F}_{\text{MLP}} \approx 168A^2 = 2.75\times 10^6$.
\begin{comment}
    \begin{equation}\label{eq:mlp_flop}
\mathcal{F}_{\text{MLP}} \approx 168A^2 = 2.75\times 10^6.
\end{equation}
\end{comment}

The \gls{hi} benchmark in~\cite{11274977} consists of an \gls{mlp}-based differential ambiguity estimator followed by a gradient-based solver. Following the parameterization in~\cite{11274977}, the total inference \gls{flop} count can be written as $\mathcal{F}_{\mathrm{HI}} \approx 7.5\times 10^4\,M + 256\,Q + 1.92\times 10^5$, where $Q$ denotes the total number of output classes of the ambiguity estimator. Since $Q$ grows linearly with $M$, the overall complexity becomes $\mathcal{O}(M)$.
\begin{comment}
    \begin{equation}\label{eq:hi_bigO}
\mathcal{O}(M).
\end{equation}
\end{comment}

\begin{comment}
    \begin{equation}\label{eq:hi_flop}
\mathcal{F}_{\mathrm{HI}}
\approx
7.5\times 10^4\,M + 256\,Q + 1.92\times 10^5,
\end{equation}
\end{comment}



%\bibliographystyle{IEEEtran}
%\nobibliography{references}

%\end{document}
